Solving reachability problems on data-aware workflows

Recent advances in the field of Business Process Management have brought about several suites able to model complex data objects along with the traditional control flow perspective. Nonetheless, when it comes to formal verification there is still the lack of effective verification tools on imperative data-aware process models and executions: the data perspective is often abstracted away and verification tools are often missing. In this paper we provide a concrete framework for formal verification of reachability properties on imperative data-aware business processes. We start with an expressive, yet empirically tractable class of data-aware process models, an extension of Workflow Nets, and we provide a rigorous mapping between the semantics of such models and that of three important paradigms for reasoning about dynamic systems: Action Languages, Classical Planning, and Model Checking. Then we perform a comprehensive assessment of the performance of three popular tools supporting the above paradigms in solving reachability problems for imperative data-aware business processes, which paves the way for a theoretically well founded and practically viable exploitation of formal verification techniques on data-aware business processes.

==> additional-backgrounds.tex <==
\section{Preliminaries} \label{app:preliminaries}

\subsection{Workflow Nets}

\begin{definition}[Petri Net~\cite{de_leoni:2013}]
  A Petri Net is a triple $\tuple{P,T,F}$ where
  \begin{itemize}
    \item $P$ is a set of places;
    \item $T$ is a set of transitions;
    \item $F\subseteq (P \times T) \cup (T \times P)$ is the flow relation describing the ``arcs'' between places and transitions (and between transitions and places).
  \end{itemize}
  
  The \emph{preset} of a transition t is the set of its input places: $\pres{t} = \{p \in P \mid (p,t) \in F\}$. The \emph{postset} of $t$ is the set of its output places: $\posts{t} = \{p \in P \mid (t,p) \in F\}$. Definitions of pre- and postsets of places are analogous.
  
  The \emph{marking} of a Petri net is a total mapping $M : P\mapsto \mathbb{N}$.
\end{definition}

\begin{definition}[WF-net~\cite{sidorovastahletal:2011}]
A Petri net $\tuple{P,T,F}$ is a workflow net (WF-net) if it has a single source place start, a single sink place end, and every place and every transition is on a path from start to end; i.e.\ for all $n\in P\cup T$, $(start,n)\in F^*$ and $(n,end)\in F^*$, where $F^*$ is the reflexive transitive closure of $F$.
\end{definition}

The semantics of a PN is defined in terms of its markings and \emph{valid firing} of transitions which change the marking. A firing of a transition $t\in T$ from $M$ to $M'$ is valid -- denoted by $M \fire{t_0} M$ -- iff:
\begin{itemize}
  \item $t$ is enabled in $M$, i.e., $\{ p\in P\mid M(p)>0\}\supseteq \pres{t}$; and
  \item the marking $M'$ satisfies the property that for every $p\in P$:
  \begin{displaymath}
    M'(p) =
    \begin{cases}
      M(p)-1 & \text{if $p\in \pres{t}\setminus\posts{t}$}\\
      M(p)+1  & \text{if $p\in \posts{t}\setminus\pres{t}$}\\
      M(p) & \text{otherwise}
    \end{cases}
  \end{displaymath}
\end{itemize}
A \emph{case} of PN is a sequence of valid firings
$$M_0 \fire{t_1} M_1, M_1 \fire{t_2} M_2, \ldots, M_{k-1} \fire{t_k} M_k$$ where $M_0$ is the marking where there is a single token in the start place.


\begin{definition}[safeness]
 A marking of a Petri Net is $k$-safe if the number of tokens in all places is at most $k$. A Petri Net is $k$-safe if the initial marking is $k$-safe and the marking of all cases is $k$-safe. 
\end{definition}

In this document we focus on 1-safeness, which is equivalent to the original safeness property as defined in~\cite{vanderaalst:1998}.\footnote{In the following we will use safeness as a synonym of 1-safeness.} Note that for safe nets the range of markings is restricted to $\{0, 1\}$.



\subsection{Action Language \klng}

The formal definition of \klng can be found in Appendix A of~\cite{eiter_dlvk:2003}; here, as reference, we include the main concepts.

We assume disjoint sets of action, fluent and type names, i.e., predicate symbols of arity $\geq 0$, and disjoint sets of constant and variable symbols. Literals can be positive or negative atoms; denoted by $-$. Given a set of literals $L$, $L^+$ (respectively, $L^-$) is the set of positive (respectively, negative) literals in $L$. A set of literals is \emph{consistent} no atoms appear both positive and negated.

The set of all action (respectively, fluent, type) literals is denoted as $\L_{act}$ (respectively, $\L_{fl}$, $\L_{typ}$). 

Furthermore, $\L_{fl,typ} = \L_{fl} \cup \L_{typ}$, $\L_{dyn} = \L_{fl} \cup \L^+_{act}$, and $\L = \L_{fl,typ} \cup \L^+_{act}$.

\begin{definition}[Causation rule]
  A (causation) rule is an expression of the form
    \begin{lstlisting}
caused $f$ if $b_1,\ldots, b_k$, not $b_{k+1}$, $\ldots$, not $b_\ell$ 
         after $a_1,\ldots, a_m$, not $a_{m+1}$, $\ldots$, not $a_n$.
  \end{lstlisting}
were $f\in \L_{fl}\cup \{ false \}$, $b_i\in\L_{fl,typ}$, $a_i\in\L$, $\ell\geq k\geq 0$ and $n\geq m\geq 0$. 

If $n=0$ the rule is called \emph{static}.

We define $h(r) = f$, $pre^+(r) = \{a_1,\ldots, a_m\}$, $pre^-(r) = \{a_{m+1},\ldots, a_n\}$, $post^+(r) = \{b_1,\ldots, b_k\}$, $post^-(r) = \{b_{k+1},\ldots, b_\ell\}$
\end{definition}



\begin{definition}[Initial state constraints]
  An initial state constraint is a static rule preceded by the keyword \lstinline|initially|.
\end{definition}

\begin{definition}[Executability condition]
  An executability condition e is an expression of the form
    \begin{lstlisting}
executable $a$ if $b_1,\ldots, b_k$, not $b_{k+1}$, $\ldots$, not $b_\ell$.
  \end{lstlisting}
were $a\in \L_{act}^+$, $b_i\in\L_{fl,typ}$, and $\ell\geq k\geq 0$.

We define $h(e) = a$, $pre^+(e) = \{b_1,\ldots, b_k\}$, and $pre^-(e) = \{b_{k+1},\ldots, b_\ell\}$
\end{definition}


Since in this document we're dealing with ground plans, for the definition of \emph{typed instantiation} the reader is referred to the original paper.

\begin{definition}[Planning domain, \cite{eiter_dlvk:2003} Def.\ A.5]
An action description $\tuple{D,R}$ consists of a finite set $D$ of action and fluent declarations and a finite set $R$ of safe causation rules, safe initial state constraints, and safe executability conditions. A \klng planning domain is a pair $PD = \tuple{\Pi,AD}$, where $\Pi$ is a stratified Datalog program (the background knowledge) which is safe, and $AD$ is an action description. We call $PD$ positive, if no default negation occurs in AD.
\end{definition}

The set $lit(PD)$ contains all the literals appearing in PD.

\begin{definition}[State, State transition]
A state w.r.t.\ a planning domain PD is any consistent set $s\subseteq\L_{fl} \cap (lit(PD) \cup lit(PD)^-)$ of legal fluent instances and their negations. A state transition is any tuple $t = \tuple{s, A, s'}$ where $s, s'$ are states and $A \subseteq \L_{act} \cap lit(PD)$ is a set of legal action instances in PD.
\end{definition}

Semantics of plans including default negation is defined by means of a Gelfond–Lifschitz type reduction to a positive planning domain.
\begin{definition}
  Let PD be a ground and well-typed planning domain, and let $t = \tuple{s,A,s'}$ be a state transition. Then, the reduction $PD^t$ of PD by $t$ is the planning domain where the set of rules $R$ of PD is substituted by $R^t$ obtained by deleting
  \begin{enumerate}
    \item each $r\in R$,where either $post^-(r) \cap s'\neq\emptyset$ or $pre^-(r)\cap s\neq\emptyset$,and
    \item all default literals \lstinline|not $\ell$| ($\ell\in\L$) from the remaining $r\in R$.
  \end{enumerate}
\end{definition}

\begin{definition}[Legal initial state, executable action set, legal state transition]
For any planning domain $PD = \tuple{D,R}$
\begin{itemize}
  \item a state $s_0$ is a legal initial state, if $s_0$ is the least set s.t.\ for all static and initial rules $r$ $post(r)\subseteq s_0$ implies $h(r) \subseteq s_0$;
  \item a set $A\subseteq\L^+_{act}$ is an executable action set w.r.t.\ a state $s$, if for each $a\in A$ there is an executability condition $e\in R^{\tuple{s,A, \emptyset}}$ s.t.\ $h(e)=\{a\}$, $pre(e) \cap \L_{fl} \subseteq s$, and $pre(e) \cap \L^+_{act} \subseteq A$;
  \item a state transition $t = \tuple{s, A, s'}$ is legal if $A$ is an executable action set w.r.t.\ $s$, and $s'$ is the minimal consistent set that satisfies all causation rules in $R^{\tuple{s,A, s'}}$ w.r.t.\ $s \cup A$. A causation rule $r \in  R^{\tuple{s,A, s'}}$, is satisfied if the three conditions
      \begin{enumerate}
        \item $post(r) \subseteq s'$
        \item $pre(r) \cap \L_{fl} \subseteq s$
        \item $pre(r) \cap \L_{act} \subseteq A$
      \end{enumerate}
      all hold, then $h(r) \neq \{false\}$ and $h(r) \subseteq s'$.
\end{itemize}
\end{definition}

\begin{definition}[Trajectory]
A sequence of state transitions $$\tuple{s_0, A_1, s_1}, \tuple{s_1, A_2, s_2}, \ldots,\tuple{s_{n-1}, A_n, s_n}$$, $n \geq 0$, is a trajectory for PD, if $s_0$ is a legal initial state of PD and all $\tuple{s_{i-1}, A_i, s_i}$, $1\leq i\leq n$, are legal state transitions of PD.

If $n = 0$, then the trajectory is empty.
\end{definition}

\begin{definition}[Planning problem]
  A planning problem is a pair of planning domain PD and a ground goal $q$
    \begin{lstlisting}
$g_1,\ldots, g_m$, not $g_{m+1}$, $\ldots$, not $g_n$.
  \end{lstlisting}
where $g_i\in\L_{ft}$ and $n\geq m\geq 0$.

A state $s$ \emph{satisfies} the goal if $\{g_1,\ldots, g_m\}\subseteq s$ and $\{g_{m+1},\ldots, g_n\}\cap s = \emptyset$.
\end{definition}

\begin{definition}[Optimistic plan]
  A sequence of action sets $A_1,\ldots, A_k$ is an optimistic plan for a planning problem $\tuple{PD, q}$ if there is a trajectory $\tuple{s_0, A_1, s_1}, \ldots,\tuple{s_{k-1}, A_k, s_k}$ establishing the goal $q$, i.e.\ $s_k$ satisfies $q$.
\end{definition}

\begin{definition}[Secure plan]
  An optimistic plan $A_1,\ldots, A_n$ is secure if for every legal initial state $s_0$ and trajectory $\tuple{s_0, A_1, s_1}, \tuple{s_1, A_2, s_2}, \ldots,\tuple{s_{k-1}, A_k, s_k}$ $0\leq k\leq n$, it holds that
  \begin{enumerate}
    \item if $k=n$ then $s_k$ satisfies the goal;
    \item if $k<n$, then there is a legal transition $\tuple{s_k,A_{k+1},s_{k+1}}$.
  \end{enumerate}
\end{definition}

\nocite{vazquez:2014,eiter_dlvk:2003}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "DataWFNets-planning.tex"
%%% save-place: t
%%% End:

==> additional-encoding-nuSMV.tex <==
%!TEX root = ./main.tex

\section{Further technical details of Section~\ref{sect:nuxmv:enc}} \label{apx:enc-nuxmv}

\thNuxmvSoundComp*

\begin{proof}
We first prove \emph{1}.
%%
Let $s'=(\mrk', \assign', t')$ be such that $s \fire{} s' \in \delta$, then we have to prove that there exists a $q'$ such that $q \fire{} q' \in \rho$ and $(s', q') \in R$. We have three cases:
\begin{compactitem}
\item $t \in T$: then, by inspecting the corresponding rule in the TRANS section, it is immediate to see that $q$ and $s$ are such that $\mrk'(p) \lra \hat{p}$ (such values are deterministic). Let us now consider the value of a generic variable $v \in \V$ assigned nondeterministically by $\assign'$: we have again three cases: either $v \in \domf(\writef(t))$ and $\writef(t)(v) \not = \emptyset$ hence its new value will be in $\writef(t)(v)$; or $\domf(\writef(t))$ and $\writef(t)(v) = \emptyset$ hence its new value will be $\udef$; or $v \not \in \domf(\writef(t))$ and its new value will be the same as the old one. Such cases are coded in conjunction in the rule: let us assume the first one applies with value $v'=c$, by Definition~\ref{def:nuxmv-ts} then there exists $q'$ such that $(q, q') \models post_i$ and $q'(v)=c$; for the other two cases the choice is deterministic, either $q'(v)=\udef$ or $q'(v)=q(v)$. It follows that there exists a $q'$ that agrees on $\enc_{\smvts}(\mrk', \assign')$. It remains to show that there exists a $q'$ such that also $q'(\hat{tr})=t'$: if $t' \in T$, then it means that $\mrk'$ and $\assign'$ satisfy the preconditions of the firing of $t'$, meaning that $t \ra \nextpre{t}$ is satisfied, hence there exists such a $q'$ (there exists at least one, the choice of $t'$ is nondeterministic); if $t'=\last$ then, from Definition~\ref{def:inf-reach-graph} we have that no $t'', \mrk'', \assign''$ such that $(\mrk', \assign') \fire{t''} (\mrk'', \assign'')$ exist, i.e., $\bigwedge_{t \in T} \neg \nextpre{t}$ holds, hence $q'(\hat{tr})=\last$. Notice that we assumed $t \in T$, hence it is never the case that $t'=\fine$. Since $q'$ agrees with $s'$ on the markings, the values of variables and the transition, it follows that $(s', q') \in R$.

\item $t=\last$, then from Definition~\ref{def:inf-reach-graph} we have that $s'=s_\epsilon$ and $t'=\fine$. Since $q(\hat{tr})=\last$, then rule $t=\last$ applies in the encoding and from its definition, $(s', q') \in R$ immediately follows.

\item $t=\fine$, then from Definition~\ref{def:inf-reach-graph} we have that $s'=s_\epsilon$ and $t'=\last$. Since $q(\hat{tr})=\fine$, then rule $t=\fine$ applies in the encoding and from its definition, $(s', q') \in R$ immediately follows.
\end{compactitem}

Now, let $q'$ such that $q \fire{} q' \in \rho$. We have to prove that there exists a $s' = (\mrk', \assign', t')$ such that $s \fire{} s' \in \delta$ and $q' = \enc_{\smvts}(\mrk', t') \land \enc_{smvts}(t)$.
We have three cases: $t \in T$, $t = \last$ and $t = \fine$. Analogous considerations of the previous case hold, as the rules in the encoding are not only sound, but also complete.


We now show \emph{2}. Given Remark~\ref{rem:enc-bijection}, it is enough to show that $(s, q) \in R$ implies $s \in S_0 \leftrightarrow q \in Q_0$.
%%
We first prove the left to right direction, i.e., that $(s=(\mrk_0, \assign_0, t), q) \in R$ implies $q \in Q_0$, namely that formula $\enc_{\smvts}(\mrk_0, \assign_0) \land \enc_{\smvts}(t)$ satisfies the first conjunct of the INIT section. By definition of INIT, the first conjunct is satisfied, thus it remains to prove $\enc_{\smvts}(t)$. By Definition~\ref{def:fin-reach-graph} and Definition~\ref{def:inf-reach-graph} either (1) $t \in T$ or (2) $t=\last$. If (1) then there is no valid firing in $(\mrk, \assign)$, which entails that $\bigwedge_{t\in T} \neg \currpre{t}$ and if (2), then $t$ can fire in $(\mrk_0, \assign_0)$ hence its preconditions are satisfied, which means $\enc_{\smvts}(\mrk_0, \assign_0)$ satisfies $\currpre{t}$. In both cases the formula in the INIT section is satisfied and $q \in Q_0$.

The right to left direction in analogous by noticing that $\currpre{}$ trivially encodes the preconditions for firing $t$.
\end{proof}





==> additional-framework.tex <==
\section{Framework}

\subsection{Data Model}\label{sec:datamodel}

\begin{definition}[Data model]
A data model for is a couple $\D = (\V, \Delta, \domf, \ordf)$ where:
\begin{compactitem}
\item $\V$ is a possibly infinite set of variables;
\item $\Delta = \set{\Delta_1, \ldots, \Delta_n}$ is a set of domains (not necessarily disjoints);
\item $\domf: \V \rightarrow \Delta$ is a total and surjective function which associate to each variable $v$ its finite domain $\Delta_i$;
\item $\ordf$ is a partial function that, given a domain $\Delta_i$, if $\ordf(\Delta_i)$ is defined, then it returns a \emph{partial order} (reflexive, antisymmetric and transitive) $\leq_{\Delta_i} \subseteq \Delta_i \times \Delta_i$.
\end{compactitem}
\end{definition}

\begin{definition}[Assignment]
Let $\D = \tuple{\V, \Delta, \domf, \ordf}$ be a data model. An assignment for variables in $\V$ is a \emph{partial} function $\assign: \V \rightarrow \Delta_v$ such that for each $v \in \V$, if $\assign(v)$ is defined, then we have $\assign(v) \in \domf(v)$. We write $\Phi[\assign]$ for the formula $\Phi$ where each occurrence of a variable $v \in \img(\assign)$ is replaced by $\assign(v)$.
\end{definition}

\begin{definition}[Guard language, syntax]
Given a data model, the language $\guardlang$ of guards is the set of formulas $\Phi$ inductively defined according to the following grammar:
\[ \begin{array}{lcl}
\Phi & := & true \mid \deff(v) \mid t_1 = t_2 \mid t_1 \leq t_2 \mid \neg \Phi_1 \mid \Phi_1 \land \Phi_2
\end{array} \]
where $v \in \V$ and $t_1, t_2 \in \V \cup \bigcup_i \Delta_i$.
\end{definition}

\begin{definition}[Guard language, semantics]
Given a data model $\dmodel$, an assignment $\assign$ and a guard $\Phi \in \guardlang$ we say that $\dmodel, \assign$ satisfies $\Phi$, written $D, \assign \models \Phi$ inductively on the structure of $\Phi$ as follows:
\begin{itemize}
\item $\dmodel, \assign \models true$;
\item $\dmodel, \assign \models \deff(v)$ iff $v \in \img(\assign)$;
\item $\dmodel, \assign \models t_1 = t_2$ iff $t_1[\assign], t_2[\assign] \not \in \V$ and $t_1[\assign] \equiv t_2[\assign]$;
\item $\dmodel, \assign \models t_1 \leq t_2$ iff $t_1[\assign], t_2[\assign] \in \Delta_i$ for some $i$ and $\ordf(\Delta_i)$ is defined and $t_1[\assign] \leq_{\Delta_i} t_2[\assign]$;
\item $\dmodel, \assign \models \neg \Phi$ iff it is not the case that $\dmodel, \assign \models \Phi$;
\item $\dmodel, \assign \models \Phi_1 \land \Phi_2$ iff $\dmodel, \assign \models \Phi_1$ and $\dmodel, \assign \models \Phi_2$.
\end{itemize} 
\end{definition}

\subsection{Petri Nets with Data}\label{sec:our-net}

\begin{definition}[\ournet] 
  A Petri Net with data is a tuple $\tuple{\dmodel, \nmodel, \writef, \guardf}$ where:
\begin{itemize}
    \item $\nmodel=\tuple{P,T,F}$ is a Petri Net;
    \item $\dmodel=\tuple{\V, \Delta, \domf, \ordf}$ is a data model;
    \item $\writef: T \mapsto (\V' \mapsto 2^{\domf(\varset)})$, where $\varset'\subseteq\varset$ and $\writef(t)(v)\subseteq\domf(v)$ for each $v\in \varset'$, is a function that associate each transition to a (\emph{partial}) function mapping variables to a subset of their domain.
    \item $\guardf: T \mapsto \guardlang$ a function that associates a guard expression to each transition.
  \end{itemize}
\end{definition}

The definition of $\writef$ provides a fine grained description of the way that transitions modify the state of the \ournet, enabling the description of different cases:
\begin{itemize}
  \item $\emptyset\subset \writef(t)(v) \subseteq \domf(v)$: transition $t$ nondeterministically assigns a value from $\writef(t)(v)$ to $v$;\footnote{Allowing a subset of  $\domf(v)$ enables the specification of restrictions for specific tasks, e.g., while a task selects among \texttt{yes, no, maybe} another one can only choose between \texttt{yes} and \texttt{no}.}
  \item $\writef(t)(v) = \emptyset$: transition $t$ deletes the value of $v$ (undefined);
  \item $v \not\in dom(\writef(t))$: value of $v$ is not modified by transition $t$.
\end{itemize}

\begin{definition}
A state of a \ournet $\tuple{\dmodel, \nmodel, \writef, \guardf}$ is a pair $(\mrk,\assign)$ where $\mrk$ is a marking for $\tuple{P,T,F}$ and $\assign$ is an assignment. State transitions and firing are adapted to the additional information about data.
\end{definition}


\begin{definition}[Valid Firing]\label{def:dpn:firing}
  Given a \ournet $\tuple{\dmodel, \nmodel, \writef, \guardf}$, a firing of a transition $t\in T$ is valid firing in $(\mrk,\assign)$ resulting in a state $(\mrk',\assign')$ (written as $(\mrk,\assign)\fire{t}(\mrk',\assign')$) iff:
  \begin{itemize}
  \item $t$ is enabled in $\mrk$, i.e., $\{ p\in P\mid \mrk(p)>0\}\supseteq \pres{t}$; and
  \item $\dmodel, \assign \models \guardf(t)$;
  \item the marking $\mrk'$ satisfies the property that for every $p\in P$:
  \begin{displaymath}
    \mrk'(p) =
    \begin{cases}
      \mrk(p)-1 & \text{if $p\in \pres{t}\setminus\posts{t}$}\\
      \mrk (p)+1  & \text{if $p\in \posts{t}\setminus\pres{t}$}\\
      \mrk (p) & \text{otherwise}
    \end{cases}
  \end{displaymath}
  \item the assignment $\assign'$ satisfies the properties that its domain is $$dom(\assign') = dom(\assign)\cup\set{v\mid \writef(t)(v)\neq\emptyset}\setminus\set{v\mid \writef(t)(v)=\emptyset}$$ and for each $v\in dom(\assign')$:
  \begin{displaymath}
    \assign'(v) =
    \begin{cases}
      d \in \writef(t)(v) & \text{if $v\in dom(\writef(t))$}\\
      \assign(v)  & \text{otherwise.}
    \end{cases}
  \end{displaymath}
\end{itemize}
\end{definition}

Cases of \ournet are defined as those of WF-nets, with the only difference that in the initial state the assignment is empty.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "DataWFNets-planning.tex"
%%% save-place: t
%%% End:


==> encoding-ASP.tex <==
%!TEX root = ./ICAPS-17-DataWFNets.tex
\section{Encoding ASP (OLD content)}
\label{sec:encoding:planning}
In this section we exploit the similarity between workflows and planning domains in order to describe the evolution of a \ournet by means of a planning language. Once the original workflow behaviour has been encoded into an equivalent planning domain, we can use the automatic derivation of plans with specific properties to solve the reachability problem.
%
In our approach we introduce a new action for each transition (to ease the description we will use the same names) and represent the status of the workflow -- marking and variable assignments -- by means of fluents.
%%
Although their representation as dynamic rules is conceptually similar we will separate the description of the encoding by considering first the behavioural part (the WF-net) and then the encoding of data (variable assignments and guards).

\subsection{Encoding \ournet behaviour}

Since we focus on 1-safe WF-nets the representation of markings is simplified by the fact that each place can either contain 1 token or no tokens at all. This information can be represented introducing a propositional fluent for each place, true iff the corresponding place holds a token.
%
Let us consider $\tuple{P,T,F}$ the \emph{safe WF-net} component of a \ournet system. The declaration part of the planning domain will include:
\begin{compactitem}
\item a fluent declaration $p$ for each place $p\in P$;
\item an action declaration $t$ for each task $t\in T$.
\end{compactitem}
Since each transition can be fired\footnote{Guards will be introduced in the next section.} only if each input place contains a token, then the corresponding action can be executed when place fluents are true: for each task $t\in T$, given $\{i^t_1, \ldots, i^t_n\} = \pres{t}$, we include the executability condition:
  \begin{lstlisting}
    executable $t$ if $i^t_1, \ldots, i^t_n$.
  \end{lstlisting}
As valid firings are sequential, namely only one transition can be fired at each step, we disable concurrency in the planning domain introducing the following rule for each pair of tasks $t_1,t_2\in T$\footnote{For efficiency reasons we can relax this constraint by disabling concurrency only for transitions sharing places or updating the same variables. This would provide shorter plans.}
  \begin{lstlisting}
    caused false after $t_1$, $t_2$.
  \end{lstlisting}
Transitions transfer tokens from input to output places. Thus the corresponding actions must clear the input places and set the output places to true. This is enforced by including  
  \begin{lstlisting}
    caused -$i^t_1$ after $t$.  $\ldots$ caused -$i^t_n$ after $t$.
    caused $o^t_1$ after $t$.  $\ldots$ caused $o^t_k$ after $t$.
  \end{lstlisting}
for each task $t\in T$ and $\{i^t_1, \ldots, i^t_n\} = \pres{t}\setminus\posts{t}$, $\{o^t_1, \ldots, o^t_k\} = \posts{t}$.
%
Finally, place fluents should be inertial since they preserve their value unless modified by an action. This is enforced by adding for each $p\in P$
  \begin{lstlisting}
    caused p if not -$p$ after $p$.
  \end{lstlisting}


\vspace{5pt}
\noindent
{\textbf{Planning problem}.} 
Besides the domain described above, a planning problem includes an initial state, and a goal.
%
In the initial state the only place with a token is the source:
  \begin{lstlisting}
    initially: $start$.
  \end{lstlisting}
%
The formulation of the goal depends on the actual instance of the reachability problem we need to solve. 
% In general it is a specific marking.
The goal corresponding to the state in which the only place with a token is $end$ is written as:
  \begin{lstlisting}
    goal: $end$, not $p_1$, $\ldots$, not $p_k$?
  \end{lstlisting}
where $\{p_1, \ldots, p_k\} = P\setminus\{ end \}$.

\subsection{Encoding data}

For each variable $v\in \varset$ we introduce a fluent unary predicate $\kvar{v}$ holding the value of that variable. Clearly, $\kvar{v}$ predicates must be functional and have no positive instantiation for undefined variables.

We also introduce auxiliary fluents to facilitate the writing of the rules. Fluent $\kvardef{v}$ indicates whether the $v$ variable is \emph{not} undefined -- it is used both in tests and to enforce models where the variable is assigned/unassigned. The fluent $\kvarchange{v}$ is used to inhibit inertia for the variable $v$ when its value is updated because of the execution of an action.

\ournet includes the specification of the set of values that each transition can write on a variable. This information is static, therefore it is included in the background knowledge by means of a set of unary predicates $\kvardom{v,t}$ as a set of facts:
  \begin{lstlisting}
    $\kvardom{v,t}$(e).
  \end{lstlisting}
  for each $v\in\varset$, $t\in T$, and $e\in \writef(t)(v)$.

\vspace{5pt}
\noindent
{\textbf{Constraints on variables}.} 
% \paragraph{Constraints on variables}
For each variable $v\in \varset$:

\begin{compactitem}
  \item we impose functionality
  \begin{lstlisting}
    caused false if $\kvar{v}$(X), $\kvar{v}$(Y), X != Y.
  \end{lstlisting}
  \item we force its value to propagate to the next state unless it is modified by an action ($\kvarchange{v}$)
  \begin{lstlisting}
    caused $\kvar{v}$(X) if not -$\kvar{v}$(X), not $\kvarchange{v}$ 
                         after $\kvar{v}$(X).
  \end{lstlisting}
  \item the defined fluent is the projection of the argument
  \begin{lstlisting}
    caused $\kvardef{v}$ if $\kvar{v}$(X).
  \end{lstlisting}
\end{compactitem}

\vspace{5pt}
\noindent
{\textbf{Variable updates}.} 
% \paragraph{Variable updates}
The value of a variable is updated by means of causation rules that depend on the transition $t$ that operates on the variable, and depends on the value of $\writef(t)$. For each $v$ in the domain of $\writef(t)$:
\begin{itemize}
  \item $\writef(t)(v) = \emptyset$: delete (undefine) a variable $v$
   \begin{lstlisting}
    caused false if $\kvardef{v}$ after t.
    caused $\kvarchange{v}$ after t.
  \end{lstlisting}
  \item $\writef(t)(v) \subseteq \domf(v)$: set $v$ with a value nondeterministically chosen among a set of elements from its domain
   \begin{lstlisting}
    caused $\kvar{v}$(V) if $\kvardom{v,t}$(V), not -$\kvar{v}$(V) after t.
    caused -$\kvar{v}$(V) if $\kvardom{v,t}$(V), not $\kvar{v}$(V) after t.
    caused false if not $\kvardef{v}$ after t.
    caused $\kvarchange{v}$ after t.
  \end{lstlisting}
   If $\writef(t)(v)$ contains a single element $d$, then the assignment is deterministic and the first three rules above can be substituted with\footnote{The deterministic version is a specific case of the non-deterministic ones and equivalent in the case that there is a single $\kvardom{v,t}(d)$ fact.}
   \begin{lstlisting}
    caused $\kvar{v}$(d) after t.
  \end{lstlisting}
\end{itemize}

\vspace{5pt}
\noindent
{\textbf{Guards}.} 
% \paragraph{Guards}
To each subformula $\varphi$ of transition guards is associated a fluent $\kguard{\varphi}$ that is true when the corresponding formula is satisfied. To simplify the notation, for any transition $t$, we will use $\kguard{t}$ to indicate the fluent $\kguard{\guardf(t)}$.
%
Executability of transitions is conditioned to the satisfiability of their guards; instead of modifying the executability rule including the $\kguard{t}$ among the preconditions, we use a constraint rule preventing executions of the action whenever its guard is not satisfied:
%
  \begin{lstlisting}
    caused false after t, not $\kguard{t}$.
  \end{lstlisting}


  Translation of atoms (\katom) is defined in terms of $\kvar{v}$ predicates. For instance $\katom(v = w)$ corresponds to \lstinline|$\kvar{v}$(V)|, \lstinline|$\kvar{w}$(W)|, \lstinline|V == W|. That is $\katom(v,T) = \kvar{t}\text{\lstinline|(T)|}$ for $t\in\V$, and $\katom(d,T) = \kvar{t}\text{\lstinline|T ==\ $d$|}$ for $d\in\bigcup_i \Delta_i$.
%
For each subformula $\varphi$ of transition guards a static rule is included to ``define'' the fluent $\kguard{\varphi}$:
\begin{tabular}{rl}
$true$ :& {\lstinline|caused $\kguard{\varphi}$ if true .|} \\
$\deff(v)$ :& {\lstinline|caused $\kguard{\varphi}$ if $\kvardef{v}$ .|} \\
$t_1 = t_2$ :& {\lstinline|caused $\kguard{\varphi}$ if $\katom$($t_1$,T1), $\katom$($t_2$,T2), T1 == T2 .|} \\
$t_1 \leq t_2$ :& {\lstinline|caused $\kguard{\varphi}$ if $\katom$($t_1$,T1), $\katom$($t_2$,T2), $\kord$(T1,T2) .|} \\
$\neg \varphi_1$ :& {\lstinline|caused $\kguard{\varphi}$ if not $\kguard{\varphi_1}$ .|} \\
$\varphi_1 \land \ldots \land \varphi_n$ :& {\lstinline|caused $\kguard{\varphi}$ if $\kguard{\varphi_1},\ldots,\kguard{\varphi_n}$ .|}
\end{tabular}
 
\subsection{Correctness and completeness}

We provide a sketch of the correctness and completeness of the encoding. Proofs can be found in~\cite{additional:ICAPS:2017}.

Planning states include all the information to reconstruct the original \ournet states. In fact, we can define a function $\plantopn{\cdot}$ mapping consistent planning states into \ournet states as following: $\plantopn{s} = (\mrk,\assign)$ with

\vspace{-.4cm}
\small
  \begin{align*}
    \forall p\in P,\; \mrk(p) = \begin{cases}
    1 \text{ if } p \in s \\
    0 \text{ otherwise}
  \end{cases} \quad
  \assign = \set{(v,d)\mid \kvar{v}(d)\in s}
  \end{align*}

\noindent  
\normalsize
$\plantopn{s}$ is well defined because $s$ it cannot be the case that $\set{\kvar{v}(d), \kvar{v}(d')}\subseteq s$ with $d\neq d'$, otherwise the static rule
  \begin{lstlisting}
    caused false if $\kvar{v}$(X), $\kvar{v}$(Y), X != Y.
  \end{lstlisting}
    would not be satisfied.
%
Moreover, 1-safeness implies that we can restrict to markings with range in $\{0,1\}$.
% \boh;{and there is not loss of information between markings and planning states.}
%%
By looking at the static rules we can observe that those defining the predicates $\kvardef{v}$ and $\kguard{t}$ are stratified. Therefore their truth assignment depends only on the extension of $\kvar{v}(\cdot)$ predicates. This implies that $\kguard{t}$ fluents are satisfied iff the variables assignment satisfies the corresponding guard $\guardf(t)$.
%%
Based on these observations, the correctness of the encoding is relatively straightforward since we need to show that a legal transition in the planning domain can be mapped to a valid firing. This is proved by inspecting the dynamic rules.
%\begin{lemma}[Correctness]\label{lemm:plantopn:correctness} Let $W$ be a \emph{safe \ournet} and $\pdom(PN)$ the corresponding planning problem. If $\tuple{s,\{t\},s'}$ is a legal transition in $\pdom(PN)$, then $\plantopn{s} \fire{t} \plantopn{s'}$ is a valid firing of $PN$.
\begin{lemma}[Correctness]\label{lemm:plantopn:correctness} Let $W$ be a \ournet and $\pdom(W)$ the corresponding planning problem. If $\tuple{s,\{t\},s'}$ is a legal transition in $\pdom(W)$, then $\plantopn{s} \fire{t} \plantopn{s'}$ is a valid~firing~of~$W$.
\end{lemma}

The proof of completeness is more complex because -- given a valid firing -- we need to build a new planning state and show that it is minimal w.r.t.\ the transition. Since the starting state $s$ of $\tuple{s,\{t\},s'}$ does not require minimality we just need to show its existence, while $s'$ must be carefully defined on the basis of the rules in the planning domain.

%\begin{lemma}[Completeness]\label{lemm:plantopn:completeness} Let $PN$ be a \emph{safe \ournet} and $\pdom(PN)$ the corresponding planning problem.
%Let $(\mrk,\assign)\fire{t}(\mrk',\assign')$ be a valid firing of $PN$, then for each consistent state $s$ s.t.\ $\plantopn{s} = M$ there is a consistent state $s'$ s.t.\ $\plantopn{s'}=M'$ and $\tuple{s,\{t\},s'}$ is a legal transition in $\pdom(PN)$.
\begin{lemma}[Completeness]\label{lemm:plantopn:completeness} Let $W$ be a \ournet, $\pdom(W)$ the corresponding planning problem and $(\mrk,\assign)\fire{t}(\mrk',\assign')$ be a valid firing of $W$. Then for each consistent state $s$ s.t.\ $\plantopn{s} = M$ there is a consistent state $s'$ s.t.\ $\plantopn{s'}=M'$ and $\tuple{s,\{t\},s'}$ is a legal transition in $\pdom(W)$.
\end{lemma}

% We briefly comment here on the construction of $s$ and $s'$. The starting state $s$ of $\tuple{s,\{t\},s'}$ does not require minimality so we just need to show its existence, while $s'$ must be carefully defined on the basis of the rules in the planning domain. 
% To simplify its characterization, $s'$ is defined as the union of the following components, which correspond to the rules providing the encoding described earlier on:
 % \scalebox{0.8}{
 % \parbox{\linewidth}{%
 %  \begin{align*}
 %    s'_{P^+} &= \set{p \in P\mid M'(p)>0} & 
 %    s'_{P^-} &= \set{-p \mid p\in \pres{t} \setminus \posts{t}} \\
 %    s'_{\varset^+} &= \set{\kvar{v}(e)\mid (v,e)\in\assign'} &
 %    s'_{\varset^-} &= \set{-\kvar{v}(e)\mid e\in\writef(t)(v), \\
 %    & & & \hspace{2.8cm} (v,e)\not\in\assign'} \\
 %    s'_{\varset^\downarrow} &= \set{\kvardef{v}\mid \kvar{v}(e)\in s'_{\varset^+}} &
 %    s'_{\varset^c} &= \set{\kvarchange{v}\mid v\in dom(\writef(t))}\\
 %    s'_{\writef} &= \set{\kvardom{v,t}(e)\mid \forall v,t,e .  &
 %    s'_{\guardf} &= \set{\kguard{t}\mid \forall t . \mrk,\assign\models\guardf(t) }\\
 %    & \hspace{2cm} e\in \writef(t)(v)}
 % \end{align*}}}

Lemmata \ref{lemm:plantopn:correctness} and \ref{lemm:plantopn:completeness}  provide the basis for the inductive proof of the following theorem:
\begin{theorem}\label{thm:wfnet:eq}
%Let $PN$ be a \emph{safe WF-net} and $\pdom(PN)$ the corresponding planning problem. Let $(\mrk_0,\assign_0)$ be the initial state of $PN$ -- i.e.\ with a single token in the source and no assignments -- and $s_0$ the planning state satisfying the initial condition.
Let $W$ be a \emph{safe WF-net} and $\pdom(PN)$ the corresponding planning problem. Let $(\mrk_0,\assign_0)$ be the initial state of $W$ -- i.e.\ with a single token in the source and no assignments -- and $s_0$ the planning state satisfying the initial condition.
 \begin{description} 
 
	 \small
 \item[$(\Rightarrow)$]
 %For \emph{any} case in $PN$
 For \emph{any} case in $W$
 \vspace{-.2cm}
  \begin{displaymath}
    \zeta: (\mrk_0,\assign_0) \fire{t_1} (\mrk_1,\assign_1) \ldots (\mrk_{n-1},\assign_{n-1})\fire{t_n} (\mrk_{n},\assign_{n})
  \end{displaymath}
  %there is a trajectory in $\pdom(PN)$
  there is a trajectory in $\pdom(W)$
  \begin{displaymath}
    \eta: \tuple{s_0,\{t_1\},s_1}, \ldots, \tuple{s_{n-1},\{t_n\},s_{n}}
  \end{displaymath}
  such that $(\mrk_i,\assign_i) = \plantopn{s_i}$ for each $i \in \{0 \ldots n\}$
  and viceversa.
  \item[$(\Leftarrow)$]
  For each trajectory
  \vspace{-.2cm}
  \begin{displaymath}
    \eta: \tuple{s_0,\{t_1\},s_1}, \ldots, \tuple{s_{n-1},\{t_n\},s_{n}}
  \end{displaymath}
   %in $\pdom(PN)$, the following sequence of firings is a  case of $PN$
   in $\pdom(W)$, the following sequence of firings is a  case of $W$
   \vspace{-.2cm}
  \begin{displaymath}
    \zeta: \plantopn{s_0} \fire{t_1} \plantopn{s_1}\ldots \plantopn{s_{n-1}} \fire{t_n} \plantopn{s_{n}}.
  \end{displaymath}
 \end{description}
\end{theorem}

Theorem~\ref{thm:wfnet:eq} above enables the exploitation of planning techniques to solve the reachability problem in \ournet. Indeed, to verify whether the final marking is reachable it is sufficient to encode it as a condition for the final state and verify the existence of a trajectory terminating in a state where the condition is satisfied.
%%
Decidability of the planning problem is guaranteed by the fact that domains are effectively finite, as in Definition~\ref{def:our-net} the $\writef$ functions range over a finite subset of the domain. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ICAPS-17-DataWFNets.tex"
%%% save-place: t
%%% End:





==> preliminaries.tex <==

\section{Preliminaries}
% \todo[inline]{Controllare che usiamo nella parte tecnica tutte queste definizioni, altrimenti levarle!}
\subsection{The Workflow Nets modeling language} % (fold)
\label{sub:subsection_name}

Petri Nets~\cite{Petri:1962aa} (PN) is a modeling language for the description of distributed systems that has widely been applied to the description and analysis of business processes~\cite{vanderaalst:1998}.%~\cite{van1995class}. 
% 
The classical PN is a directed bipartite graph with two node types, called \emph{places} and \emph{transitions}, connected via directed arcs. Connections between two nodes of the same type are not allowed. 

\begin{definition}[Petri Net]
	\label{def:PN}
  A \emph{Petri Net} is a triple $\tuple{P,T,F}$ where $P$ is a set of \emph{places}; $T$ is a set of \emph{transitions}; $F\subseteq (P \times T) \cup (T \times P)$ is the flow relation describing the arcs between places and transitions (and between transitions and places).
\end{definition}
The \emph{preset} of a transition $t$ is the set of its input places: $\pres{t} = \{p \in P \mid (p,t) \in F\}$. The \emph{postset} of $t$ is the set of its output places: $\posts{t} = \{p \in P \mid (t,p) \in F\}$. Definitions of pre- and postsets of places are analogous.
Places in a PN may contain a discrete number of marks called tokens. Any distribution of tokens over the places, formally represented by a total mapping  $M : P\mapsto \mathbb{N}$, represents a configuration of the net called a \emph{marking}.  
%

\begin{figure}
  \centering
    \fbox{\includegraphics[width=.35\linewidth]{imgs/PNsample.pdf}}
  \caption{A Petri Net.}
  \label{fig:imgs_PNsample}
\end{figure}
PNs come with a graphical notation where places are represented by means of circles, transitions by means of rectangles and tokens by means of full dots within places. Figure~\ref{fig:imgs_PNsample} depicts a PN with a marking $M(p_0)=2$, $M(p_1)=0$, $M(p_2)=1$. The preset and postset of $t$ are $\{p_0, p_1\}$ and $\{p_2\}$, respectively.  



\begin{figure*}[h]
  \centering
    % \includegraphics[width=.5\textwidth]{imgs/SampleWFnet.pdf}
    \tikzstyle{place}=[circle,draw=black,thick]
    \tikzstyle{transition}=[text width=2cm,text centered,rectangle,draw=black!50,fill=black!20,thick]
    \scalebox{0.6}{\begin{tikzpicture}[font=\large]
      \node (start) [place,label=above:$start$] {};
      % \node at ( 0,1) [place] {};
%       \node at ( 0,0) [place] {};
      \node[transition,text width=2cm] (t1)  [right=.5cm of start, anchor=west] {T1:ask application documents};
      \node[place,label=right:$p_1$] (p1) [right=.8cm of t1, anchor=west] {};
      \node[transition] (t2)  [above right=1.5cm of p1, anchor=west] {T2:send student application};
      \node[transition] (t3)  [below right=1.5cm of p1, anchor=west] {T3:send worker application};
      \node[place,label=above:$p_2$] (p2) [right=.5cm of t2] {};
      \node[place,label=below:$p_3$] (p3) [right=.5cm of t3] {};
      \node[transition] (t4)  [right=.5cm of p2, anchor=west] {T4:fill student request};
      \node[transition] (t5)  [right=.5cm of p3, anchor=west] {T5:fill worker request};
      \node[place,label=left:$p_4$] (p4) [right=8cm of p1, anchor=west] {};
      \node[transition,text width=3cm] (t6)  [above right=2cm of p4] {T6:local credit officer approval};
      \node[transition,text width=3cm] (t7)  [right=1.3cm of p4] {T7:senior credit officer approval};
      \node[transition,text width=3cm] (t8)  [below right=2 cm of p4] {T8:bank credit committee approval};
      \node[place,label=above right:$p_5$] (p5) [right=5.5cm of p4, anchor=west] {};
      \node[transition,text width=.5cm] (t9)  [right=.5cm of p5] {T9};
      \node[place,label=above:$p_6$] (p6) [above=1cm of t9] {};
      \node[place,label=below:$p_7$] (p7) [below=1cm of t9] {};
      \node[transition] (t10)  [right=1cm of p6] {T10:send approval to customer};
      \node[transition] (t11)  [right=1cm of p7] {T11:store approval in branch};
      \node[place,label=above:$p_8$] (p8)  [right=1cm of t10] {};
      \node[place,label=below:$p_9$] (p9)  [right=1cm of t11] {};
      \node[transition,text width=1.5cm] (t12)  [below=.8cm of p8] {T12: issue loan};
      \node[place,label=above:$end$] (end)  [right=.5cm of t12] {};
      \draw [->,thick] (start.east) -- (t1.west);
      \draw [->,thick] (t1.east) -- (p1.west);
      \draw [->,thick] (p1.north) to [bend left=45] node[fill=white,inner sep=1pt, near start] {{loanType=s}} (t2.west);
      \draw [->,thick] (p1.south) to [bend right=45] node[fill=white,inner sep=1pt, near start, swap] {{loanType=w}} (t3.west);
      \draw [->,thick] (t2.east) to (p2.west);
      \draw [->,thick] (t3.east) to (p3.west);
      \draw [->,thick] (p2.east) to (t4.west);
      \draw [->,thick] (p3.east) to (t5.west);
      \draw [->,thick] (t4.east) to [bend left=45] (p4.north);
      \draw [->,thick] (t5.east) to [bend right=45] (p4.south);
      \draw [->,thick] (p4.north) to [bend left=45] node[fill=white,inner sep=1pt, midway] {{request$\leq 5k$}} (t6.west);
      \draw [->,thick] (p4.south) to [bend right=45] node[fill=white,inner sep=1pt, midway,swap] {{request$\geq 100k$}} (t8.west);
      \draw [->,thick] (p4.east) to node[fill=white,inner sep=1pt, midway,swap] {else} (t7.west);
      \draw [->,thick] (t6.east) to [bend left=45] (p5.north);
      \draw [->,thick] (t8.east) to [bend right=45] (p5.south);
      \draw [->,thick] (t7.east) to  (p5.west);
      \draw [->,thick] (p5.east) to (t9.west);
      \draw [->,thick] (t9.north) to (p6.south);
      \draw [->,thick] (t9.south) to (p7.north);
      \draw [->,thick] (p6.east) to (t10.west);
      \draw [->,thick] (p7.east) to (t11.west);
      \draw [->,thick] (t10.east) to (p8.west);
      \draw [->,thick] (t11.east) to (p9.west);
      \draw [->,thick] (p8.south) to  (t12.north);
      \draw [->,thick] (p9.north) to  (t12.south);
      \draw [->,thick] (t12.east) to  (end.west);
    \end{tikzpicture}}
  \caption{A process as a Petri Net.}
  \label{fig:imgs_SampleWFnet}
\end{figure*}	
% The idea of using Petri Nets to model processes starts from the observation that business processes are basically ordered set of tasks. Thus they can be mapped onto a Petri Net in the following way: tasks are modeled by transitions and precedence relations are modeled by places.
%%
Process tasks are modeled in PNs as transitions while arcs and places constraint their ordering.
%%
For instance, the process in Figure~\ref{fig:imgs_SampleWFnet}\footnote{For the sake of simplicity we only focus here on the, so-called, happy path, that is the successful granting of the loan.}
% Consider, for instance, the process of a \emph{Loan Request} depicted in Figure~\ref{fig:imgs_SampleWFnet}\footnote{For the sake of simplicity we only focus here on the, so-called, happy path, that is the successful granting of the loan}. The 10 tasks that compose the process are modeled by transitions. This process
exemplifies how PNs can be used to model parallel and mutually exclusive choices, typical of business processes: sequences \emph{T2;T4}-\emph{T3;T5} and transitions \emph{T6-T7-T8} are indeed placed on mutually exclusive paths. Transitions \emph{T10} and \emph{T11} are instead placed on parallel paths. Finally, \emph{T9} is needed to prevent connections between nodes of the same type. 


The expressivity of PNs exceeds, in the general case, what is needed to model business processes, which typically have a well-defined starting point and a well-defined ending point. This imposes syntactic restrictions on PNs, that result in the following definition of a workflow net (WF-net)~\cite{vanderaalst:1998}.
%DECISO CON SERGIO DI LASCIARE PERDERE FREE-CHOICE. COMPLICATO DA CAPIRE E NON CI SERVE.
% 
\begin{definition}[WF-net]
A PN $\tuple{P,T,F}$ is a WF-net if it has a single source place $start$, a single sink place $end$, and every place and every transition is on a path from start to end, i.e., for all $n\in P\cup T$, $(start,n)\in F^*$ and $(n,end)\in F^*$, where $F^*$ is the reflexive transitive closure of $F$.
\end{definition}

A marking in a WF-net represents the \emph{workflow state} of a single case. The semantics of a PN/WF-net, and in particular the notion of \emph{valid firing}, defines how transitions route tokens through the net so that they correspond to a process execution. 

\begin{definition}[Valid Firing]
	\label{def:Firing}
A firing of a transition $t\in T$ from $M$ to $M'$ is \emph{valid}, in symbols $M \fire{t} M'$, iff
\begin{enumerate}
  \item $t$ is enabled in $M$, i.e., $\{ p\in P\mid M(p)>0\}\supseteq \pres{t}$; and
  \item the marking $M'$ is such that for every $p\in P$:
  \begin{displaymath}
	  \small
    M'(p) =
    \begin{cases}
      M(p)-1 & \text{if $p\in \pres{t}\setminus\posts{t}$}\\
      M(p)+1  & \text{if $p\in \posts{t}\setminus\pres{t}$}\\
      M(p) & \text{otherwise}
    \end{cases}
  \end{displaymath}
\end{enumerate}
\end{definition}
Condition 1.~states that a transition is enabled if all its input places contain at least one token; 2.~states that when $t$ fires it consumes one token from each of its input places and produces one token in each of its output places. 

A \emph{case} of a WF-Net  is a sequence of valid firings 
$M_0 \fire{t_1} M_1, M_1 \fire{t_2} M_2, \ldots, M_{k-1} \fire{t_k} M_k$ 
where $M_0$ is the marking indicating that there is a single token in $start$.

\begin{definition}[$k$-safeness]
 A marking of a PN is $k$-safe if the number of tokens in all places is at most $k$. A PN is $k$-safe if the initial marking is $k$-safe and the marking of all cases is $k$-safe.
\end{definition}
From now on we concentrate on $1$-safe nets, which generalize the class of \emph{structured workflows} and are the basis for best practices in process modeling~\cite{kiepuszewskihofstedeetal:2013}. We also use safeness as a synonym of 1-safeness. 
% For safe nets the range of markings is restricted to $\{0, 1\}$.
It is important to notice that our approach can be seamlessly generalized to other classes of PNs, as long as it is guaranteed that they are $k$-safe. This reflects the fact that the process control-flow is well-defined (see~\cite{heesidorovaetal:2003}).


% Figure~\ref{fig:imgs_PNsample} depicts a WF-Nets model focused on the so-called control-flow perspective and ignores data associated with the different cases. However, the decisions to be taken in actual executions of this procedure highly depend on characteristics of the loan request (e.g., the size of the loan) and of the house (e.g., its structural status). The need to incorporate the data-flow into WF-Nets has originated some proposals for extending WF-Nets with the ability to manipulate data~\cite{sidorovastahletal:2011,de_leoni:2013}. The main idea of these approaches is to consider data elements (e.g., High liability) that can be used on transitions' pre-conditions, a language for composing these data elements into boolean guards, and (read/write) operations that specify how transitions operate on data elements.


% \begin{definition}[safeness]
%  A marking of a Petri Net is $k$-safe if the number of tokens in all places is at most $k$. A Petri Net is $k$-safe if the initial marking is $k$-safe and the marking of all cases is $k$-safe. 
% \end{definition}

% In this document we focus on 1-safeness, which is equivalent to the original safeness property as defined in~\cite{vanderaalst:1998}.\footnote{In the following we will use safeness as a synonym of 1-safeness.} Note that for safe nets the range of markings is restricted to $\{0, 1\}$.
% subsection subsection_name (end)

\vspace{5pt}
\noindent
{\textbf{Reachability on Petri Nets}.} The behavior of a PN  can be described as a transition system where states are markings and directed edges represent firings. Intuitively, there is an edge from $M_i$ to $M_{i+1}$ labeled by $t_i$ if $M_i \fire{t} M_{i+1}$
is a valid firing. Given a ``goal'' marking $M_g$, the reachability problem amounts to check if there is a path from the initial marking $M_0$ to $M_g$. Reachability on PNs (WF-nets) is of enormous importance in process verification as it allows for checking natural behavioral properties, such as satisfiability and soundness in a natural manner~\cite{Aalst97}.
%%

\subsection{Trace repair} % (fold)
\label{sub:trace_repair}

One of the goals of process mining is to capture the  as-is  processes  as  accurately  as  possible: this is done by examining event logs that can be then exploited to perform % process discovery, conformance checking, and process enhancement, as graphically 
the tasks in Figure~\ref{fig:imgs_ProcessMiningTypes}. In many cases, however, event logs are subject to data quality problems, resulting in \emph{incorrect} or \emph{missing} events in the log. In this paper we focus on the latter issue addressing the problem of \textbf{repairing execution traces that contain missing entries} (hereafter shortened in trace repair).  

The need for trace repair is motivated in depth in~\cite{Rogge-Solti2013}, where missing entities are described as a frequent cause of low data quality in event logs, especially when the definition of the business processes integrates activities that are not supported by IT systems due either to their nature (e.g. they consist of human interactions) or to the high level of abstraction of the description, detached from the implementation. A further cause of missing events are special activities (such as transition \emph{T9} in Figure~\ref{fig:imgs_SampleWFnet}) that are introduced in the model to guarantee properties concerning e.g., the structure of the workflow or syntactic constraints, but are never executed in practice. 
% Second, IT systems may expose only partial information about their workings and the data they produce, hence preventing a complete execution tracing.

The starting point of trace repair are \emph{execution traces} and the knowledge captured in \emph{process models}. Consider for instance the model in Figure~\ref{fig:imgs_SampleWFnet} and the (partial) execution trace 
% \begin{equation}
% \label{eq:trace-nodata}
\{T3, T7\}.
% \end{equation}
By aligning the trace to the model using a replay-based approach or a planning based approach, the techniques presented in~\cite{Rogge-Solti2013} and~\cite{Di-Francescomarino-C.:2015aa} are able to exploit the events stored in the trace and the control flow specified in the model to reconstruct two possible repairs: 

\scalebox{0.9}{
\parbox{\linewidth}{%
\begin{align*}
\label{eq:trace-complete-nodata1}
\{T1, T3, T5, T7, T9, T10, T11, T12 \} \\
% \label{eq:trace-complete-nodata2}
\{T1, T3, T5, T7, T9, T11, T10, T12 \}
\end{align*}
}}

Consider now a different scenario in which the partial trace reduces to \{$T7$\}. In this case, by using the control flow in Figure~\ref{fig:imgs_SampleWFnet} we are not able to reconstruct whether the loan is a student loan or a worker loan. This increases the number of possible repairs and therefore lowers the usefulness of trace repair. Assume nonetheless that the event log conforms to the XES standard and stores some observed data attached to $T7$ (enclosed in square brackets): 
\begin{equation*}
\label{eq:trace-data}
\{T7[request=\cvalue{60k},loan=\cvalue{50k}]\}
\end{equation*}
If the process model is able to specify how transitions can read and write variables, and furthermore some constraints on how they do it, the scenario changes completely. Indeed, assume that transition \emph{T4} is empowered with the ability to write the variable $request$ with a value smaller or equal than $\cvalue{30k}$ (being this the maximum amount of a student loan). Using this fact, and the fact that the request examined by \emph{T7} is greater than $\cvalue{30k}$, we can understand that the execution trace has chosen the path of the worker loan. Moreover, if the model specifies that variable \emph{loanType} is written during the execution of \emph{T1}, when the applicant chooses the type of loan she is interested to, we are able to infer that \emph{T1} sets variable \emph{loanType} to $\cvalue{w}$. 
This example, besides illustrating the idea of trace repair, also motivates why data are important to accomplish this task, and therefore why extending repair techniques beyond the mere control flow is a significant contribution to address data quality problems in event logs.  
% subsection trace_repair (end)

\subsection{The planning language \klng} % (fold)
\label{sub:planning_language}
The main elements of action languages are \emph{fluents} and \emph{actions}. The former represent the state of the system which may change by means of actions. Causation statements describe the possible evolution of the states, and preconditions associated to actions describe which action can be executed according to the current state.
A planning problem in \klng~\cite{eiter_dlvk:2003} is specified using a Datalog-like language where fluents and actions are represented by literals (not necessarily ground). The specification includes the list of fluents, actions, initial state and goal conditions; also a set of statements specifies the dynamics of the planning domain using causation rules and executability conditions.
%
The semantics of \klng borrows heavily from Answer Set Programming (ASP) paradigm. In fact, the system enables the reasoning with partial knowledge and provides both weak and strong negation.

A \emph{causation rule} is a statement of the form
\begin{lstlisting}
    caused $f$ if $b_1$,$\ldots$, $b_k$, not $b_{k+1}$, $\ldots$, not $b_\ell$ 
               after $a_1$,$\ldots$, $a_m$, not $a_{m+1}$, $\ldots$, not $a_n$.
\end{lstlisting}
%where $f$ is either a classical literal over a fluent or \texttt{false} (representing absurdity), the $b_i$s are classical literals (atoms or strongly negated atoms, indicated using \texttt{-}) over fluents and background predicates and the $a_j$s are positive action atoms or classical literals over fluent and background predicates.
 The rule states that $f$ is true in the new state reached by executing (simultaneously) some actions, provided that $a_1,\ldots,a_m$ are known to hold while $a_{m+1},\ldots,a_n$ are not known to hold in the previous state (some of the $a_j$ might be actions executed on it), and $b_1,\ldots,b_k$ are known to hold while $b_{k+1},\ldots,b_\ell$ are not known to hold in the new state.
 %
 Rules without the \lstinline|after| part are called \emph{static}.

An \emph{executability condition} is a statement of the form
\begin{lstlisting}
    executable $a$ if $b_1$,$\ldots$, $b_k$, not $b_{k+1}$, $\ldots$, not $b_\ell$.
\end{lstlisting}
%where $a$ is an action atom and $b_1,\ldots,b_\ell$ are classical literals (known as pre-conditions in the statement).
 Informally, such a condition says that the action $a$ is eligible for execution in a state, if $b_1,\ldots,b_k$ are known to hold while $b_{k+1},\ldots,b_\ell$ are not known to hold in that state.

Terms in both kind of statements could include variables (starting with capital letter) and the statements must be safe in the usual Datalog meaning w.r.t.\ the first fluent or action of the statements.

%
%Additionally, \klng provides some macros to express commonly used patterns. These are internally expanded using the above two statements together with strong and weak negation.
%%
%For example a fluent can be declared \texttt{\textbf{inertial}}, expressing the fact that its truth value does not change unless explicitly modified by an action, or it could be stated that after an action there should be total knowledge concerning a given fluent. For more details the reader should refer to~\cite{Eiter:2003qf}.

A \emph{planning domain PD} is a tuple $\tuple{D,R}$ where $D$ is a finite set of action and fluent declarations and $R$ a finite set of  rules, initial state constraints, and executability conditions.

The semantics of the language is provided in terms of a transition system where the states are ASP models (sets of atoms) and actions transform the state according to the rules. A state transition is a tuple $t = \tuple{s, A, s'}$ where $s, s'$ are states and $A$ is a set of action instances. The transition is said to be legal if the actions are executable in the first state and both states are the minimal ones that satisfy all causation rules. Semantics of plans including default negation is defined by means of a Gelfond-Lifschitz type reduction to a positive planning domain.
%
A sequence of state transitions $\tuple{s_0, A_1, s_1}, \ldots,\tuple{s_{n-1}, A_n, s_n}$, $n \geq 0$, is a trajectory for PD, if $s_0$ is a legal initial state of PD and all $\tuple{s_{i-1}, A_i, s_i}$, are legal state transitions of PD.

A \emph{planning problem} is a pair of planning domain PD and a ground goal
\lstinline|$g_1,\ldots, g_m$, not $g_{m+1}$, $\ldots$, not $g_n$.|
% \end{lstlisting}
that is required to be satisfied at the end of the execution.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ICAPS-17-DataWFNets"
%%% save-place: t
%%% End:
